A Generalised Inverse Reinforcement Learning Framework

The gloabal objective of inverse Reinforcement Learning (IRL) is to estimate the unknown cost function of some MDP base on observed trajectories generated by (approximate) optimal policies. The classical approach consists in tuning this cost function so that associated optimal trajectories (that minimise the cumulative discounted cost, i.e. the classical RL loss) are 'similar' to the observed ones. Prior contributions focused on penalising degenerate solutions and improving algorithmic scalability. Quite orthogonally to them, we question the pertinence of characterising optimality with respect to the cumulative discounted cost as it induces an implicit bias against policies with longer mixing times. State of the art value based RL algorithms circumvent this issue by solving for the fixed point of the Bellman optimality operator, a stronger criterion that is not well defined for the inverse problem. To alleviate this bias in IRL, we introduce an alternative training loss that puts more weights on future states which yields a reformulation of the (maximum entropy) IRL problem. The algorithms we devised exhibit enhanced performances (and similar tractability) than off-the-shelf ones in multiple OpenAI gym environments.

==> Src-commit/Experiments_deprecated_ICML.tex <==
\section{Experiments}
\label{sec:experiments}
    This section is devoted to experimental evidences that $\MEGAN$ achieves state of the art performances. It is compared to GAIL as all subsequent approaches build upon its formulation.
    In both the simple and multi-task settings, the considered environments come with a true cost function that we used to learn an expert behaviour using SAC. The obtained policy is then used to generate the expert trajectories. 
    
    When sampling transitions for the discriminator, the canonical approach is to use a uniform distribution\footnote{This is possible since used trajectories are always finite.} over the horizon to reduce the bias against policies with longer mixing times. We use this scheme for the implementation of GAIL.
    However, for the sampling procedure of MEGAN, we respect the theoretical propositions. We use a discount factor $\gamma=0.995$ (which makes $\rho_\pi$ a long term predictive future state distribution), and we use $\eta=\Geom(0.7)$ (which makes $P_\pi^\eta$ a short term predictive future state distribution). This way, MEGAN carries a long-short term interpretation: it mimics the short term behaviour in sub-trajectories initialised in states encountered on the long term behaviour in trajectories initialised according to~$p_0$.
    
    
    \subsection{Simple task setting}
        In this section we consider both the \hbox{\textit{Hopper}} and the \hbox{\textit{Walker}} environments from the \hbox{\textit{PyBullet Gymperium}} package \cite{pybullet_gym}. 
        We evaluate MEGAN (without the Idle generator procedure) and GAIL using the same expert data set and the same hyper-parameters\footnote{From a practical point of view, the implementation of both algorithms is the same except for the sampling procedure. This implies that there is no confounding parameters in play.}. We compare normalised costs of the best performing policies in both cases and provide a random behaviour performance as a baseline.
        
        \begin{figure}[ht]
        \centering
            \includegraphics[width=.9\linewidth]{Figure/Test_performances_single.png}
            \caption{Normalised cumulative costs in the single-task setting}
            \label{single_task}
        \end{figure} 
        
        On Figure \ref{single_task}, we provide the box-plots of normalised cumulative costs in $1000$ runs of the best performing policies. 
        We observe that both GAIL and MEGAN provide comparable average performances. However, the GAIL policy has a much more consistent/robust learned behaviour (as illustrated  by the absence of outliers, especially in the \hbox{\textit{Walker}} environment). This is explained by the fact that MEGAN matches future state occupancy measures even for trajectories initialised in states visited over extended horizons (in trajectories initialised according to $p_0$). 
            
    \subsection{Multi-task setting}
        Classically, the multi-task setting is defined by considering a task space $\Theta$ and for each task $\theta\in\Theta$ the associated Markov decision process \hbox{$\mathcal{M}_\theta=\{\mathcal{S}, \mathcal{A}, \mathcal{P}, c_\theta, \gamma, p_0\}$}. Depending on the context, the objective
     is then to either solve the RL or the IRL problems for the set of MDPs $(\mathcal{M}_\theta)_{\theta\in\Theta}$ by averaging the losses with respect to a task distribution $\mathcal{F}$.
        This is equivalent in principle to solving the problem for the MDP \hbox{$\Bar{\mathcal{M}}=\{\mathcal{S}\times\Theta, \Bar{\mathcal{A}}, \Bar{\mathcal{P}}, \Bar{c}, \gamma, \Bar{p}_0\}$} where for any states $(s,s')$, tasks $(\theta,\theta')$ and action $a$:
        \begin{align*}
            &\Bar{\mathcal{A}}(s,\theta)  &= & \; \mathcal{A}(s) & \\
            &\Bar{\mathcal{P}}(s',\theta'|s,\theta,a) &  = & \; \mathcal{P}(s'|s,a)\delta(\theta'=\theta)&\\
            &\Bar{c}(s,\theta,a) & = & \; c_\theta(s,a) & \\
            &\Bar{p}_0(s,\theta) & = & \; p_0(s)\mathcal{F}(\theta) &
        \end{align*}
        We adapt the latter formulation here for the sake of coherence with previous sections. 
        We consider in the remaining of this section the \hbox{\textit{FetchReach}}\footnote{To the extent of our knowledge, this is the first reported performances of IRL algorithms on a fully continuous environment} task from the \textit{MuJoCo} based environments \cite{mujoco_gym}.  
        To evaluate the generalisability of the learned policies, we only generate expert trajectories for a subset of possible tasks (only target positions that are $5$-$10$ cm away from the initial gripper's position\footnote{the maximum range of the arm is about $25$ cm} to be precise). We evaluate the learned policies in the \textit{learned setting} (same horizon and same tasks) and in a \textit{generalisability setting} (twice the training horizon and the full range of tasks). As in the simple task setting, we asses performances in terms of normalised cumulative costs.
        
        
        The difficulty in multi-task settings arises from ray-interference: when the cost function encourages conflicting behaviours for different tasks, the learning objective plateaus \cite{ray_interference}. This stagnates the progress of the policy, which in turn complicates the IRL problem as these plateaus are an opportunity for the discriminator to over-fit the replay-buffer. To alleviate this issue, we propose to \textit{augment the data-set} as proposed in Section \ref{sec:data_augmentation} (by using $\MEGAN$ coupled with the Idle subroutine (Algorithm \ref{A:Idle_On_policy})).
          
        \begin{figure}
       \centering
            \begin{subfigure}{.49\linewidth}
                \includegraphics[width=\linewidth]{Figure/Learning_performances_multi_task.png}
                \caption{Normalised cumulative costs over training}
                \label{multi_task_learning}
            \end{subfigure}
            \begin{subfigure}{.46\linewidth}
                \includegraphics[width=.9\linewidth]{Figure/Test_performances_multi_task.png}
                \caption{Normalised cumulative costs (best performance)}
                \label{multi_task}
            \end{subfigure}
            \caption{Performances in the Fetch Reach setting}
            \label{multi-task}
        \end{figure} 
        
        In Figure \ref{multi_task_learning}, we compare the performances of MEGAN (with and without the data augmentation) and GAIL over the training. We observe that both GAIL and MEGAN (without Idle) struggle in solving the problem. However, using the Idle generator reduces the undesirable effect of ray interference and stabilises the training.
        Performance wise, the learned policy using MEGAN outperforms the expert demonstrations in the training tasks while at the same time providing comparable performances in the remaining set of tasks (as provided in Figure \ref{multi_task}).
        
        
        It is arguable that the success of MEGAN in the multi-task setting is explained with the Idle procedure. A similar approach on GAIL might be appealing. However, this is not feasible in practice.
        It is true that the reasoning provided in Section \ref{sec:data_augmentation} can be developed for any distribution $\eta$, this entails that we can use the same approach to learn a generator that mimics $\rho_\pi(.|s_0)$. Unfortunately, this is not feasible in practice (due to the high variance of $\rho_\pi$, as explained in Section \ref{sec:data_augmentation}). The issue at play here is that the latter distribution ($\rho_\pi)$ covers all the observations of the trajectory. Indeed, from our early empirical attempts, we noticed that learning such distribution is unstable: we either over-fit a sub-set of the trajectory (notably the stationary distribution, which is hurtful for our purpose) or we do not learn the distribution at all. 
        On the other hand, learning $P_\pi^\eta$ conditioned on some intermediate state is a lot easier when we choose $\eta$ such that it only covers the near future transitions (for example when $\eta=\Geom(0.7)$, the average prediction of $P_\pi^\eta(|s_t)$ is $3$ steps in the future). 
        
        In Figure \ref{idle_samples}, we evaluate the learned approximation of $P_{\pi_E}^{\Geom(0.7)}$ on a sample expert trajectory. We plot the evolution of  the (true/generated) gripper position in 3D overtime.  For each state encountered on the trajectory, the learned generator outputs $10$ samples (in blue). Clearly, the future state generator is reliable; this is successful because the distribution $\eta$ is a short term prediction: the learned generator maps current states to the possible ones in the next few steps. 
            
        \begin{figure}[ht]
        \centering
            \includegraphics[width=\linewidth]{Figure/Idle example.png}
            \caption{Idly generated samples from expert trajectory}
            \label{idle_samples}
        \end{figure}     
        
        Additional experimental results on a fully continuous multi-task $2$-D navigation environment with similar conclusions are reported in Appendix \ref{A:experiments} .
        
        %to either \textit{pre-process the expert trajectories} (by using an expert data set of trajectories that mainly focuses on the pre-mixing phase\footnote{as opposed to the stationary distribution (for example, the part of the trajectory before reaching the goal in the \textit{FetchReach} environment.) }) \textbf{or} to 
        
       
        
        %\subsubsection*{Pre-processing the expert data-set:}
        %    From our early empirical attempts, we noticed that when the expert trajectories are mainly observations from the stationary phase of the behaviour (i.e. when the robotic gripper is hovering around the target task), the discriminator ends up over-fitting this phase and the task of learning the policy becomes extremely difficult. 
            
        %    By cutting the speed of simulations to a third in the \hbox{\textit{FetchReach}} environment, and only sampling expert target positions (tasks) that are $5$ to $10$ cm away from the initial position of the gripper\footnote{the maximum range of the arm is about $25$ cm}, we obtained a homogeneous pre-mixing time across possible demonstrations (between $20$ and $25$ time steps before reaching the position). The data set of expert demonstrations is composed of trajectories with a horizon of $50$ transitions.
            
        %   {\color{blue}FIGURE + PERFORMANCE}
            
        %    However, this approach is environment specific and requires an understanding of the underlying cost function. 
            
        %\subsubsection*{Data augmentation}

==> Src-commit/rebutal.tex <==
We thank the reviewers for their constructive feedbacks and quality reviews. We identified three main concerns. Due to length constrains we will answer them collectively.
%while including indications in the form of [\#reviewer ID] to help them navigate the rebuttal easily. 
We also provide an ablation analysis of the distribution $\eta$.

\textbf{Motivating the proposed problem [1,5,6]:}
    Given an MDP, the Bellman optimality criterion optimises Q-values for any state-action pairs (discounted rewards only optimises initial state values). This is why value-based RL outperforms  policy-based one in many cases. However, this operator is not well-defined for the IRL problem with respect to the cost function, hence the   issues with longer horizons. 
    Our criterion bridges this gap.\\
    It optimises weighted Q-values along the expert trajectory: by choosing $\small \eta=\Geom(\gamma)$, the criterion becomes the sum of discounted Q-values. %[1]. 
    Notice that adding $\eta$ does not affect alignment with value-based RL as it converges to $\eta$-optimal policies (c.f.\ Corollary~\ref{PR:opt_reg_policy}). %~[5]. 
    Hypothetically, there could be other generalisations of discounted rewards. However, preserving the Bellman optimality criterion for RL and duality properties for the IRL isn't trivial (using a polynomial decay $\frac{\gamma}{t^n}$ breaks this). An interesting alternative is using GAIL with $\gamma=1$ in finite horizons. This case is to be compared with $\gamma,\eta=1$ for MEGAN. We provide empirical evidence in the next section to prove that the latter is better.\\ 
    We also agree that $(\pi_E, \frac{1}{2})$ is a Nash equilibrium of the  game between  agent and  discriminator for any choice of $\eta$ (including the classical case). However, this does not imply at all that the learning dynamic will converge to that particular pair % due to approximation errors and the non-stability of this equilibriu
    (Idle -a GAN model- suffers from the same issue: Algorithm \ref{A:Idle_On_policy} can fail despite Proposition \ref{P:Idle}). 
    A more probable equilibrium is $(\RL(\Tilde{c}), \Tilde{c}=\IRL(\pi_E))$. This is further confirmed empirically, as the learned cost function isn't uniform (cf Appendix \ref{A:experiments}). For such equilibrium, the choice of the criterion is crucial for the ability to match both $\rho_{\pi_E}$ and $\mu_{\pi_E}$.  %[6].
    This is confirmed in the provided new ablation analysis~of~$\eta$.

\textbf{Questions regarding the $\eta$ Distribution [All]:}
    Intuitively, our criterion is considering `$\eta$-future' states that the policy reaches if it was to start from `$\gamma$-future' states, themselves reached from the initial state distribution .\ This entails from Proposition \ref{tower_rule}.\ It also relates to the long-short term interpretation from the experiences. %~[1].
    In the paper we only used geometric distributions as it guarantees duality property (c.f.\ Proposition \ref{PR:equivalent}). However, choosing other distributions is perfectly possible (weak duality properties are guaranteed in the IRL and no effect on value-based RL). \\
    In order to address the issue concerning the choice of $\eta$, we provide a new ablation analysis. % as requested by the reviewers.   %[5,6].
    We evaluate the divergence between the expert and the learned occupancy measures ($(\rho_{\Tilde{\pi}}, \rho_E)$ and $(\mu_{\Tilde{\pi}}, \mu_E)$ with $\tiny \gamma,\eta=.99$). 
    We use the MMD divergence between samples from the expert data and the replay buffer obtained during training. This procedure evaluates performances across the policies toward which the algorithm converges, while factoring in their stability.\\
    For a better diversity, we use yet another environment: Half-Cheetah. We use MEGAN to train $\Tilde{\pi}$ with different parameters of geometric distributions (we point out that $\eta=0$ is a Dirac mass, and $\eta=1$ is a uniform distribution) as-well as different parameters of the Poisson distribution. In all experiments, we use $\gamma=1$ to highlight the importance of using $\eta$ in the learning process. We also point out that the used hyper-parameters are selected based on the literature and not on a fine-tuning procedure. This is advantageous for GAIL as previous works adapted these parameters for it. 
    What is striking about the Figure is that despite the weaker theoretical guarantees for non geometric distribution, using a Poisson distribution with parameter $25$, achieved the lowest divergence to the expert data-set. Notably, $25$ frames is, on average, a Half-Cheetah movement cycle that repeats it-self. As if our choice of $\eta$ built in an inductive bias within MEGAN. Notice how with $\eta$ as a uniform, we achieve similar performances. % [All]. 

\textbf{Questions regarding sampling \& Idle[All]:}
    We start by pointing out that sampling from $\mu$ (for any given $\eta$) is easy when using on-policy trajectories (c.f.\ Section \ref{sec:tractability}). Proposition \ref{tower_rule} guarantees that inverting the order of sampling $\gamma/\eta$-future states does not cause discrepancies between equations and algorithms. %[1].
    However, learning $\mu/\rho$ using Idle is hard mainly due to mode collapse (c.f.\ Appendix \ref{A:experiments}).\\ To circumvent this issue, we proposed to only learn $P^\eta$ and couple it with sampling according to $\rho$ (c.f.\ L5 in Algorithm \ref{Algo:Megan}). Notice that using Idle with GAIL can be done in one of two ways: either try to learn directly $\rho$ which will fail, or try to learn a $P^{\delta_0}$ which is strictly equivalent to a simple instance of GAIL. This is why using Idle in the Multi-task setting is only useful when combined with MEGAN. To highlight this fact, we propose to evaluate the divergence between occupancy measures using MEGAN+Idle while varying the parameter $\eta$. The results are accurately predicted by the reviewer. % [5].
    
    
    \begin{figure}[ht]
        \centering
            \includegraphics[width=.9\linewidth]{Figure/rebuttal.png}
            \caption{Evidence of MMD minimisation under $\eta$-optimality}
            \label{rebuttal}
    \end{figure} 
